Veritas: Answering Causal Queries from Video Streaming Traces

In this paper, we seek to answer what-if questions - i.e., given recorded data of an existing deployed networked system, what would be the performance impact if we changed the design of the system (a task also known as causal inference). We make three contributions. First, we expose the complexity of causal inference in the context of adaptive bit rate video streaming, a challenging domain where the network conditions during the session act as a sequence of latent and confounding variables, and a change at any point in the session has a cascading impact on the rest of the session. Second, we present Veritas, a novel framework that tackles causal reasoning for video streaming without resorting to randomised trials. Integral to Veritas is an easy to interpret domain-specific ML model (an embedded Hidden Markov Model) that relates the latent stochastic process (intrinsic bandwidth that the video session can achieve) to actual observations (download times) while exploiting control variables such as the TCP state (e.g., congestion window) observed at the start of the download of video chunks. We show through experiments on an emulation testbed that Veritas can answer both counterfactual queries (e.g., the performance of a completed video session had it used a different buffer size) and interventional queries (e.g., estimating the download time for every possible video quality choice for the next chunk in a session in progress). In doing so, Veritas achieves accuracy close to an ideal oracle, while significantly outperforming both a commonly used baseline approach, and Fugu (an off-the-shelf neural network) neither of which account for causal effects.

==> Zdag.tex <==
\section{Causal Graph}
%\begin{figure*}
%    \includegraphics[width=\textwidth]{figs/design-confounder.png}
%    \caption{Examples of real-world causal DAGs and implications in video streaming.}
%    \label{fig:design-confounder}
%\end{figure*}
\textbf{Key terms:} 

\begin{itemize}
%    \item \textbf{Causal reasoning}: answering \textit{'what-if'} questions, given data obtained from a real world deployment of existing system.
%    \item \textbf{Counterfactual reasoning}: queries about past sessions.
    \item \textbf{Confounder}: Consider three variables X, Y and Z. If X influences Y, but Z influences both X and Y, Z is a confounder, because it introduces a correlation/dependence between X and Y even in the absence of a direct connection between X and Y. ~\cite{sruthi2020netai}  \item \textbf{Latent confounder}: Require capturing dynamic network state. Ex: bandwidth, latency, etc.
    \item \textbf{Observable confounder}: Available in datasets. Ex: type of connection, chunk size, etc.
\end{itemize}

\textbf{Key ideas:}

\begin{itemize}
    \item Derive Causal Dependency Graphs for Internet content and video delivery applications.
    \item Develop models to use the observed variables to get the latent variables and answer \textit{'what-if'} questions.
\end{itemize}

\begin{itemize}
    \item Explaining DAGs in video streaming:
    A framework for answering counterfactual questions involves using causal graphs (DAGs). DAGs identifies the variables in a system and their causal relationships. We need to identify from a DAG whether an adjustment is needed to identify causal effect, if yes, find minimum set of variables (\textit{backdoor variables} to isolate the causal effect. Focusing on video streaming, which involves splitting video into chunks, each encoded at multiple qualities. Adaptive Bit Rate (ABR) algorithms~\cite{mpc,pensieve,oboe,BBR,bola} decide which quality to download each chunk in a manner that balances multiple video delivery metrics such as the video quality, quality variations, rebuffering, and delays at user join time. Video performance is known to impact user engagement (e.g., how long a user stays in the video session)~\cite{QOEModelSigcomm13,SitaramanCausalityIMC12,conviva-sigcomm2011}. 
    
    \item Explaining possible biases: For instance, \ref{fig:design-confounder}(a) illustrates an example in the context of video streaming, where a spurious correlation between content length, and video quality may arise owing to the time of day acting as a confounding variable. For instance, users may watch longer entertainment videos at night when performance in home networks also happens to be poorer, while shorter news/business clips are viewed during the day. \ref{fig:design-confounder}(b) which shows that the choice of resolution can impact rebuffering, while both video resolution and the extent of rebuffering impact how long a user stays. 
    \ref{fig:design-confounder}(c) presents a preliminary version of the dependencies to be considered, which we will refine as our research evolves. We will also extend our models to consider temporal aspects (since each variable may be observed over different time steps), as well as more complex scenarios where the video session may download
    chunks from multiple CDNs, which in turn may be chosen based on
    observed performance~\cite{ghabashnehexploring,c3}. With these graphs, we identify variables to adjust on using the techniques discussed above, and develop appropriate causal adjustments. One challenge is that the ground truth bandwidth is a latent variable, for which a proxy may not be readily available. 
    
    \begin{figure}[h]
        \includegraphics[width=0.48\textwidth]{figs/design-cdg.pdf}
        \caption{\bruno{Show why (MIT paper) task is simplified with d-separation}\small{Modeling dependencies in an ABR algorithm}}
        \label{fig:design-cdg}
    \end{figure}
    
    \item Latent confounders: Many video streaming systems rely on predicting throughput~\cite{cs2p}, which can help an Adaptive Bit Rate (ABR) algorithm decide what quality to choose for each chunk.
    However, as we and other researchers~\cite{bartulovic_biases_2017,xatuSigmetrics22} have pointed out, the throughput observed by an ABR algorithm depends on its size (since small-sized chunks may encounter TCP slow start effects), an important aspect not widely considered~\cite{cs2p,mpc}.
    Most recently, Xatu~\cite{xatuSigmetrics22}
    (developed by us), and Fugu~\cite{yan_learning_2020} have attempted to correct for these effects through observational ML models trained on data from previous video sessions which explicitly consider size. Both these works involve neural networks that predict the download time of a video chunk given its size, and given the size and the download times of the previous $K$ chunks.
    
\end{itemize}


==> Zevaluation.tex <==
\section{Evaluation}
In this section, we evaluate \System{} with respect to how effectively it can respond to causal queries (what-if questions) when given traces collected from a video streaming system. Our evaluations focus on both kinds of causal queries:

\noindent
$\bullet$ \textbf{Counterfactual queries.} Given traces collected from a video streaming system with a particular set of design decisions, we evaluate the effectiveness of \System{} when  answering what-if questions related to the performance of the system on \textit{the same set of traces} if one could go back in the past and use a new set of decisions. The decisions that we consider include
(i) changing the set of video qualities that the streaming algorithm may choose
from; (ii) changing the buffer size available to the video player; and (iii)
changing the underlying ABR algorithm itself.

\noindent
$\bullet$ \textbf{Interventional queries.} Given traces collected from a video 
streaming algorithm, we evaluate the effectiveness of \System{} on answering what-if questions related to the system on a new set of traces collected in similar environments. Specifically, we compare the effectiveness of \System{} in predicting download times of video chunks of Algorithm B although only trained on traces collected from the deployment of Algorithm B. \sgr{Weak? May not convey the idea that
associational approach is basically useless in practice.}

\textbf{Schemes compared.}
We compare \System{} with two approaches: 

\noindent
$\bullet$ \textbf{Ground Truth (\GT{}):} This refers to the ground truth bandwidth, defined in \S\ref{sec:causalDAG}. When answering
what-if questions, results using this technique serve as the ideal benchmark, that \System{} and other approaches must seek to 
achieve.  

\noindent
$\bullet$ \textbf{\Baseline{}:} This scheme directly use the observed throughput of each chunk, and assumes this throughput value holds from the start time of the chunk download to the end time of download. During off periods when no estimate is available, linear interpolation of the throughput observed by the previous and next chunks is used. The scheme is commonly used in most video streaming evaluations today. It is expected to be a more accurate representation when the observed throughput is close to \capacity{}, but underestimates otherwise, and may be inaccurate during off-periods. \sgr{note: MIT paper uses a weaker baseline.} 

\textbf{Evaluation setup.}

\begin{figure}[h]
    \includegraphics[width=8cm]{figs/evaluation-design.png}
    \caption{Evaluation setup}
    \label{fig:eval-setup}
\end{figure}

When evaluating counterfactual questions, we use the evaluation
setup shown in Figure~\ref{fig:eval-setup}. \sgr{Chandan, please add a figure}:
Consider that we have logs from a video streaming session in
Setting A, and we wish to understand the performance if Setting B were used.

\noindent
$\bullet$ First, we run a video streaming session in Setting A emulating a ground truth network bandwidth trace. This results in a log which for each chunk includes (i) size; (ii) start time of download; and (iii) end time of download.

\noindent
$\bullet$ Next, we post-process the log above using \Baseline{} and \System{} which results in an inference of \Capacity{} traces
from each of these techniques. 

\noindent
$\bullet$ We next run the video streaming session in Setting B using
the \Capacity{} traces inferred by \System{} and \Baseline{}, as well as the original \Capacity{} trace.

\noindent
While \Baseline{} only returns a single reconstruction of \Capacity{},
\System{} allows for sampling to capture the inherent uncertainty of the inference process. Unless otherwise mentioned, we sample 5 \sgr{Fix when finalized} \Capacity{} traces from \System{}, each of which represents a possible reconstruction of \Capacity{} that \System{} deems feasible. We emulate the video streaming session in Setting B with each of the traces and \System{} responds to each what-if query with a range of 
potential outcomes.

\textbf{Evaluation metrics.} In our counterfactual questions, we compare the result predicted by each of \System{}, \Baseline{}, and \GT{} with respect to the actual what-if scenario. Our counterfactual questions pertain to the impact of a change on the quality of a video session. Hence, we use standard metrics such as video quality (measured by the SSIM), rebuffering ratios, and change of SSIM. We also report a QoE metric that combines these measures. \sgr{Improve.} Our interventional questions pertain to prediction accuracies of chunk download times.

%\begin{itemize}
%    \item Deployment: We use FCC traces for network bandwidth and run MPC to stream video with N=3 qualities. The video data is collected as used as a baseline for deployed ABR, and potential what-if question.
%    \item What-if: We add better qualities (three new) for the video and check the performance of the MPC ABR.
%    \item Comparison: Baseline traces, HMM decoded traces and ground truth.
%\end{itemize}

%The difference between what-if-baseline and what-if-true is the basis of the evaluation and scope of improvement.


\textbf{Setup details.}
\sgr{Chandan, please expand}.
\begin{itemize}
    \item Mahimahi: We use the emulation setup used by Fugu ~\cite{yan_learning_2020}, which involved emulating traces using Mahimahi ~\cite{mahimahi}, and a 10 minute pre-recorded video clip in three qualities. The clients are launched inside a mahimahi shell with a 80 ms end to end delay and downlink GTBW limited by FCC traces.
    \item Emulation of FCC traces: We use FCC traces with GTBW within 3 to 8 Mbps. This upper limit of GTBW is more than sufficient to watch the video in highest quality.
    \item HMM trained on tridiagonal matrix: The transition matrix used by eHMM is a tridiagonal matrix. It priortizes the GTBW to be stable, but it can vary by transitioning through various GTBW states over time.  
    \item TCP training set: For our throughput estimator, we set up an emulation environment with a server and client. The client runs in a mahimahi shell and receives payloads of different sizes [2KB to 4 MB] from the server with random intervals of wait time [0.12 to 8s] between successive payloads. The GTBW of mahimahi shell is varied from 0.5 to 10 Mbps, and the end to end delay is varied from 5 to 40 ms using mahimahi.
    \item MPC default algorithm, 5 sec buffer: We use the MPC ABR ~\cite{mpc} implemented in Puffer with a buffer of 5s and rebuffering coefficient of 100 for video streaming in our setup, unless mentioned otherwise.
\end{itemize}


\subsection{Counterfactuals with \System{}: Example}


\begin{figure*}[!htb]
\centering
\subcaphangtrue
\subfigcapmargin = .09cm
\subfigure[GTBW and Baseline for an example trace.]{
\includegraphics[width=0.75\textwidth]{figs/example-whatif-step-1.png}
\label{fig:what-if-step-1}
}
\subfigure[GTBW and Veritas samples for an example trace.]{
\includegraphics[width=0.75\textwidth]{figs/example-whatif-step-2.png}
\label{fig:what-if-step-2}
}
\caption{\small{Comparing Baseline, GTBW and Veritas samples for an example trace.}}
\vspace{-0.07in}
\label{fig:example-what-if}
\end{figure*}
   
%*HMM model: set of 100 FCC traces from 0 to 10Mbps avg bandwidth.
%*Deployment used 50 traces from 9 to 10 Mbps (40 completed). Ran MPC


Consider that the video streaming application has been deployed with a given set of video qualities. The designer wishes to ask what would happen if the qualities were increased.


\sgr{Chandan: TODO: find a good figure to show and add here. ideally has a more certain and less certain region.} 
\cb{Using a trace for MPC, LMH instead of low quality to high quality. We might need to alter the order of questions.}
Figure~\ref{fig:what-if-step-1} illustrates the \Capacity{} seen during the session for an example trace, as well as the performance observed by \Baseline{}. \Baseline{} is conservative in its estimation of \Capacity{} since for the lower qualities used in the deployment, the observed throughput tends to be significantly lower than \Capacity{}.

Figure~\ref{fig:what-if-step-2} illustrates the time series reconstructed by \System{}. Several potential candidates that are deemed likely are revealed by \System{}, and we show 5 sample traces. We make several observations. First, all these traces are closer to \Capacity{} than \Baseline{}. Second, there are regions that \System{} is relatively more certain, where all sample traces are close to \Capacity{}. However, there are other regions where it is relatively less certain, and \System{} indicates a range of possibilities. This occurs because if the chunk sizes selected by the deployed algorithm are close to the bandwidth delay product (BDP) or higher, the observed throughput is closer to \Capacity{}, and \System{} is relatively more certain. If however the chunk sizes are smaller, a range of different \Capacity{} values may have resulted in the same throughput observations, and \System{} is less certain. Note also that \System{}'s use of HMMs allows it to sample more likely transition regions from the less certain to more certain regions.



\begin{figure*}[!htb]
\centering
\subcaphangtrue
\subfigure[SSIM for example trace.]{
\includegraphics[width=0.22\textwidth]{figs/example-ssim.png}
\label{fig:example-ssim}
}
\subcaphangtrue
\subfigure[Rebuffering for example trace]{
\includegraphics[width=0.22\textwidth]{figs/example-rebuf.png}
\label{fig:example-rebuf}
}
\subcaphangtrue
\subfigure[SSIM for change of ABR.]{
\includegraphics[width=0.22\textwidth]{figs/change_abr_sorted_ssim.png}
% \caption{}
\label{fig:change-abr-ssim}
}
\subfigure[Rebuffering for change of ABR.]{
\includegraphics[width=0.22\textwidth]{figs/change_abr_sorted_rebuf.png}
\label{fig:change-abr-rebuf}
% \caption{Rebuffering for chnage of ABR.}
}
\subcaphangtrue
\subfigure[SSIM for change of buffer size.]{
\includegraphics[width=0.22\textwidth]{figs/change_buffer_sorted_ssim.png}
\label{fig:change-buffer-ssim}
% \caption{}
}
\subfigure[Rebuffering for change of buffer size.]{
\includegraphics[width=0.22\textwidth]{figs/change_buffer_sorted_rebuf.png}
\label{fig:change-buffer-rebuf}
% \caption{}
}
\subfigure[SSIM for change of qualities.]{
\includegraphics[width=0.22\textwidth]{figs/change_quality_sorted_ssim.png}
\label{fig:change-quality-ssim}
% \caption{}
}
\subfigure[Rebuffering for change of qualities.]{
\includegraphics[width=0.22\textwidth]{figs/change_quality_sorted_rebuf.png}
\label{fig:change-quality-rebuf}
}
\vspace{-0.07in}
\caption{\small{Comparing SSIM and rebuffering ratio for counterfactual queries.}}
\vspace{-0.07in}
\label{fig:change-metrics}
% \caption{Rebuffering for change of ABR.}
\end{figure*}

Figure~\ref{fig:example-metrics} presents the result of the what-if analysis query for rebuffering ratio, and video quality (measured by SSIM). \sgr{One or two graphs which show rebuf ratio and SSIM for baseline, ground truth, and each of our samples for this example trace.}

Next, we show results on repeating our analysis for all 100 traces. For each trace, when we run the what-if query, we run 5 samples with \System{}, and consider the minimum and maximum \sgr{XX or 2nd lowest and 2nd largest?}. We call each of these \SystemLow{} and \SystemHigh{}.



Figure~\ref{fig:example-metrics} presents the distribution of the SSIM and rebuffering ratio observed across the traces with each of the schemes. We make several observations. First, \Baseline{} is quite far away from \GT{}. Second, \GT{} lies in between \SystemLow{} and \SystemHigh{}, and the range is relatively small.

Slide 14. SSIM, Rebuf. SSIM consistently higher.
            

*time series for MPC to BBA,
*MPC to BBA
*Change of buffer
*Change of quality -> 5 more runs
*time permits, analyze MPC-> BOLA (less critical)

\subsection{Diverse counterfactual questions}

\noindent
\textbf{Change of buffer size.}
We next consider the counterfactual question: what would be the impact of changing the buffer size. In this case, we consider that the video streaming application has been deployed with an ABR and a chosen buffer size. The designer then wants to know the impact of increasing the buffer size. Intuitively, increasing the buffer size should increase the performance of the ABR. A larger buffer protects the player against rebuffering events and also provides more degrees of freedom to optimise performance ~\cite{mpc}. In our case, the deployments consists of MPC ABR with initial buffer size of 5s and we evaluate the performance if the buffer size were to be increased to 30s. We see in Figure~\ref{fig:change-buffer-metrics}, the GTBW sees no rebuffering events and the SSIM values are high (close to 0.985). However, Baseline observes rebuffering and estimates lower SSIM. Veritas performs better than baseline and has no rebuffering and observes SSIM values close to GTBW.


Slide 12 Rebuf, SSIM
Digging in: 
  *Some examples where Baseline predicts high rebuf. Why does it happen?
  
  


\noindent
\textbf{Change of algorithm.}
We next consider the counterfactual: what would have been the impact of using a different ABR algorithm. The designer uses MPC and wants to use BBA ~\cite{tysigcomm2014} in future. We use the BBA implemented in Puffer setup ~\cite{yan_learning_2020}. It uses the formula in the original paper to decide the maximum chunk size, and subject to this constraint, the chunk with the highest SSIM is selected to stream. The buffer size for both MPC and BBA is 5s. To reinforce the aggressive nature of BBA, we choose an upper reservoir value of 0.95.

We see in ~\ref{fig:change-abr-metrics} that Veritas observes SSIM and rebuffering close to GTBW. However, baseline estimates much lower SSIM and higher rebuffering. 


%What-if questions that we ask:
%\begin{itemize}
   % \item Moved from 3 lowest qualities to 3 highest qualities (40 traces) [9-10] [5 sec buffer]
    %\item Two qualities. Upgrade lower quality to a better one, but keep higher one the same. (13 traces)
    %        [3-8Mbps] [5 sec buffer]
    %\item Change the buffer size - but keep the video qualities the same.
    %        Same details as below, but change buffer size to 30 secs.
    %\item Change the ABR algorithm - keep the video qualities the same. Deployment has 3: L/M/H.
    %      RTT is 80 ms. L: median is 30 KB, 95\%ile is 87 KB; H: (1 MB, 2.3 MB). H has avg of 4.1 Mbps.
    %          5 sec buffer [3 - 8 Mbps]
    %\item Same ABR, but turn off TCP slow-start restart \sgr{Not sure.}
    %\item Change from TCP cubic to TCP BBR (not sure if we can do this - lower on our stack now).
%\end{itemize}


\subsection{Interventional queries: bias-free download time prediction}
We next consider the ability of \System{} to answer interventional queries that relate to the future (\S\ref{sec:background}), focusing on the ability to
predict chunk download times in a bias-free fashion.
 
%Some ABRs use Neural networks (NN) to predict the download time of chunks and use it to choose the video quality of the chunk to be sent. However, using NN could lead to inherent bias in the prediction of download time as shown in Fig \ref{fig:fugu-bias}.
%Our set up consists of:

We compare two schemes:

\noindent $\bullet$ \textbf{FuguNN:} This refers to a neural network proposed in \cite{yan_learning_2020} which predicts the download time of chunks based on the sizes and download times of prior chunks. While the approach is effective at predicting chunk download times for the deployed ABR, it suffers from a bias when predicting download times for a new ABR as shown in \S\ref{XX}.
%It predicts the probability distribution over 21 bins of  download time: [0,0.25),[0.25,0.75),[0.75,1.25),...,[9.75, $\infty$)s. For simplicity, we use only download time and sizes of past chunks as inputs to FuguNN.

\noindent
$\bullet$ \textbf{\System{} + CapNN:}
Rather than chunk sizes and download times, we create a neural network trained on ground truth bandwidth traces \sgr{IMPORTANT: people may ask how we can obtain it, or if OK}.
Using only the chunks downloaded upto a particular point in the session, we use \System{} to infer multiple samples of the \Capacity{} time series for the past, from which we derive
an average \Capacity{} time series. We then use the above neural network to predict the next \GT{} value in the sequence, and then using our model predict observed throughput for the next chunk.


~\cb{$\bullet$ \textbf{\System{}}: Using only the chunks downloaded upto a particular point in the session, we use \System{} to infer \Capacity{} time series for the past. In this case, we use Viterbi coding to get \Capacity{} trace. We use the tridiagonal transition matrix from eHMM to get the expected value of \capacity{} for next chunk and then using our throughput estimator predict the observed throughput for the next chunk.}
    
%CapNN: We propose a NN which uses the hidden variable, capacity, as input and predicts the probability distribution of network capacity over 35 bins: [0, 0.5), [0.5, 1), ... [16.5, $\infty$) Mbps. As part of video streaming data, we do not have the network capacity information (hidden state) for the chunks. However, we have the observations such as cwnd, ssthresh, throughput, etc. for past chunks and we can use our HMM to get the hidden variable, network capacity, which is then fed to CapNN. Finally, we use network capacity from the output of CapNN together with throughput estimator to get the download time of chunks. In both, CapNN and FuguNN, we estimate the output to be the midpoint value of the bin with maximum probability.

    
%\begin{figure}[h]
%\includegraphics[width=8cm]{figs/exp-bias-distribution.png}
%\caption{Distribution of chunk sizes and download times.}
%\label{fig:exp-bias-distribution}
%\end{figure}
      
    \begin{figure}[h]
        \centering
        \includegraphics[width=4cm]{figs/final-hmm-fugu-lmh-scatter.png}
        \caption{Comparing FuguNN and HMM for download time prediction \sgr{Replace with new result. \cb{Done}}}
        \label{fig:exp-fugu-bias-result}
    \end{figure}

\sgr{Need to revise from here on.}
We run video streaming sessions using MPC as ABR over the FCC traces. These video streams are then used to train FuguNN and CapNN. To simplify the setup, we use two qualities: High and Low; and two network conditions: high bandwidth (9-10 Mbps) and low bandwidth (0 to 0.3 Mbps). The distribution of download time and chunks sizes in shown in Fig. \ref{fig:exp-bias-distribution}.
  
To compare the performance of the two NN's and get the actual download time of video chunks [choice of video chunk not influenced by ABR], we choose the video chunks of video streams randomly and measure the download time.

The results are shown in Fig. \ref{fig:exp-fugu-bias-result}
    



==> Zmodel_f.tex <==
%
\paragraph{Domain-inspired emission model.}
% \label{subsec:model_f}

% A video chunk can observe $Y_n$ close to ~\Capacity{} if $S_n$ is greater than network bottleneck characterised by the Bandwidth-Delay Product (BDP)~\cite{BBR}. We use the given \Capacity{} and minimum RTT from the TCP state $W_{s_n}$ to calculate $BDP$.  We consider a simple model, ~\ModelF with  an Additive Increase - Multiplicative Decrease (AIMD) congestion control mechanism with slow start. We consider TCP Slow Start Restart (TCP SSR) ~\cite{ssr} based on ~\cite{ssr-algo} and Linux kernel TCP implementation. If the time since last packet send ($W_{s_n}^{last\_send}$) is greater than the retransmission time out ($W_{s_n}^{rto}$), TCP SSR is triggered and the congestion window ($W_{s_n}^{cwnd}$) and slow start threshold ($W_{s_n}^{ssthresh}$) are updated which can limit the throughput observed by a video chunk. Possible scenarios include: (i) $W_{s_n}^{cwnd}$ $>$ $S_n$ and $S_n$ $>$ BDP: the chunk will observe $Y_n$ close to \Capacity{}. (ii) $W_{s_n}^{cwnd}$ $>$ $S_n$ and $S_n$ $<$ $BDP$: it will take one transmission round to send the chunk. (iii) $W_{s_n}^{cwnd}$ $<$ $S_n$: We estimate the number of rounds required to transmit the chunk using Additive Increase of $W_{s_n}^{cwnd}$. 


The throughput ($Y_n$) observed by video chunk $n$ is a function of \Capacity{} ($C_{s_n},\ldots,C_{e_n}$), the starting TCP state $W_{s_n}$, and the chunk size ($S_n$). \bruno{something about only $C_{s_n}$} We develop a general model, ~\ModelF to estimate $Y_n$ based on Additive Increase - Multiplicative Decrease (AIMD) congestion control with slow start and slow start restart (TCP SSR)  ~\cite{ssr}. ~\ModelF does not model loss events and simplifies the evolution of congestion window. If the network is idle and ($W_{s_n}^{last\_send}$) is greater than the retransmission time out ($W_{s_n}^{rto}$), TCP SSR is triggered and the congestion window ($W_{s_n}^{cwnd}$) and slow start threshold ($W_{s_n}^{ssthresh}$) are updated according to Linux kernel implementation based on ~\cite{ssr-algo}. We calculate the number of transmission rounds needed to transmit a chunk with size $S_n$ based on the updated $W_{s_n}^{cwnd}$ and $W_{s_n}^{ssthresh}$. We then use minimum RTT in $W_{s_n}$, the number of transmission rounds and $S_n$ to estimate the observed throughput by the video chunk. We test the performance of \ModelF in an emulation environment with a server transmitting payloads of different sizes [2KB to 4 MB] to a client, with random intervals of wait time [0.12 to 8s] between transmission of successive payloads. ~\ModelF derives $W_{s_n}$ using the socket stats utility in Linux~\cite{ss}. The ~\Capacity{} between client and server is varied from 0.5 to 10 Mbps, and the end to end delay is varied from 5 to 40 ms using mahimahi ~\cite{mahimahi} across experiments. The GTBW and delay is kept constant for a particular experiment. \Cref{fig:f_accuracy} shows a CDF of the relative error between the actual throughput observed by a payload and the throughput estimated by~\ModelF across all \Capacity{} and delays. In most cases, the predicted throughput is within a range of 1 Mbps of the observed throughput by the payload. 

\sgr{Chandan: Moving model evaluation here. Can you make things flow, and also write some text on the relative error?}
\begin{figure}[t]
    \centering
    \includegraphics[width=5cm]{figs/error_tcp_video.png}
    \caption{Relative error of ~\ModelF{}.\gao{Chandan, we need a breif explanation of this plot.}}
    \label{fig:f_accuracy}
\end{figure} 

% \begin{algorithm}
% \caption{Network throughput estimator}
% \hspace*{\algorithmicindent} \textbf{Input} {Network capacity (C), congestion window (cwnd), slow start threshold (ssthresh), minimum RTT (min\_rtt), RTO (rto), time since last send (last\_snd), chunk size (size)} \\
% \hspace*{\algorithmicindent} \textbf{Output} {Chunk throughput (Y)} 

% \begin{algorithmc}
% \Procedure{f}{C, cwnd, ssthresh, min\_rtt, rto, last\_snd, size}


% \end{algorithmc}

% \end{algorithm}

==> Zmotivation.tex <==
\section{Causal Challenges in Video Streaming}

% We need to add background for each point. May be a subsection.


Our work is motivated by following observations in Internet Video Streaming:

\begin{enumerate}[itemsep=0.05pt]
  %\item Video streaming today typically involves splitting video into chunks, each encoded at multiple bitrates. Clients pick bitrates for each chunk so as to balance between achieving high video quality, while avoiding rebuffering based on network conditions. Several Adaptive Bitrate (ABR) algorithms ~\cite{bb,bola,mpc,festive,tian,pensieve, oboe} have emerged to tackling this challenge. However, the design of these algorithms is complicated by the fact that clients must predict chunk download times, a challenging problem ~\cite{cs2p}. 
  
  \item An obvious fix to the above problem would be to predict throughput instead of download time. However, throughput is dependent on the size of chunks: a larger size chunk will see higher throughput and smaller size chunk will see lower throughput. Thus, only throughput estimation will not help in identifying the network condition.
  
  \item For argument sake, let us assume we were able to make the throughput estimation size agnostic. However, throughput itself is dependent on network state. We use ~\cite{mahimahi} to simulate a fixed bandwidth of 18 Mbps between a client and server. Then, we send payloads of varying size (2 KB to 4 MB) between client and server. We observe the throughput at client side. In ~\ref{fig:throughput-variance}, we see that throughput is dependent on size (as explained before) and also depends on network state (explained in system design).
  
%   \vspace{-12pt}
  \begin{figure}[h]
    \includegraphics[width=8cm]{figs/motivation-throughput.png}
    \caption{Variance in throughput for a fixed bandwidth (18 Mbps) depending on network state.}
    \label{fig:throughput-variance}
  \end{figure}
%   \vspace{-8pt}

  %\item Most of the video streaming ABRs use existing video streaming session data for evaluation. This creates an inherent bias in the ABR model based on the original ABR which was running when the data was collected. [Need to elaborate or rethink on this.]
  


\end{enumerate}

==> Zsystem_design.tex <==
\section{System Design}












==> acknowledgements.tex <==
We thank Cloudlab ~\cite{cloudlab} for providing us with the computing resources to run the emulation experiments.

==> methoddescription.tex <==
\section{Causal Machine Learning for Video Streaming}

One of the key contributions of our work is the **definition of the task**.
We start by giving a definition for {\em interventional learning}, which we refined from Mitchell's definition of learning \cite[Chapter 1.1]{Mitchell1997}. Given
\begin{enumerate}
    \item a video delivery task over an unseeing session with a new method,
    \item training experience (existing recorded sessions) obtained with an old method, and
    \item a performance measure,
\end{enumerate}
a computer program is said to {\em learn video delivery interventions} if its performance in the new method at the task improves if give more experience (existing recorded sessions with old method).

We can further refine the above to give a definition of {\em counterfactual inference for *video streaming*}. Given
\begin{enumerate}
    \item training experience (existing recorded sessions) running an old streaming method, 
    \item a new method, and
    \item a performance measure,
\end{enumerate}
a computer program is said to perform {\em counterfactual inference} if it can evaluate the performance of the new method if it had been used in the existing recorded sessions where the old method was used.


==> my_math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,amsthm,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\Puni}{{\bm{P}}}


\newcommand{\indep}{\perp \!\!\! \perp }

\newcommand{\doop}{\text{do}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}

\newtheorem{definition}{Definition}
\newtheorem{proposition}{Proposition}
\newtheorem*{proposition*}{Proposition}
\newtheorem{theorem}{Theorem}
\newtheorem*{theorem*}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem*{corollary*}{Corollary}
\newtheorem{remark}{Remark}
\newtheorem{lemma}{Lemma}
\newtheorem*{lemma*}{Lemma}

\newcommand{\bcH}{\mathcal{H}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cO}{\mathcal{O}}

% --------------------------------------------------------------------------- %
% Reduce vertical spacing of \dbar

\makeatletter
\let\overlinewithoriginalheight\overline
\newcommand*\overlinewithlessheight[1]{{\mathpalette\overline@aux{#1}}}
%% N.B. extra {} is necessary for (mostly) proper superscript height
\newcommand*\overline@aux[2]{% %% #1 = \displaystyle etc., #2 = actual arg.
  \begingroup
    \count0=\fam %% Store the font (e.g. \mathbf)
    \setbox0=\hbox{$\m@th #1\fam=\count0 #2$}% %% just to measure #2
    \@tempdima=.4\ht0% %% Store 0.4 * height of #2
    \setbox0=\hbox{$\m@th #1\fam=\count0\overlinewithoriginalheight{#2}$}%
    \advance\@tempdima by .6\ht0% %% Add .6 * height of \overline{#2}
    \ht0=\@tempdima %% set ht of box 0 to .4 * ht(#2) + .6 * ht(\overline{#2})
    \usebox0% %% print box 0
  \endgroup%
}
\let\overline\overlinewithlessheight

\let\underlinewithoriginaldepth\underline
\newcommand*\underlinewithlessdepth[1]{{\mathpalette\underline@aux{#1}}}
\newcommand*\underline@aux[2]{%
  \begingroup
    \count0=\fam
    \setbox0=\hbox{$\m@th #1\fam=\count0 #2$}%
    \@tempdima=.4\dp0%
    \setbox0=\hbox{$\m@th #1\fam=\count0\underlinewithoriginaldepth{#2}$}%
    \advance\@tempdima by .6\dp0%
    \dp0=\@tempdima
    \usebox0%
  \endgroup%
}
\let\underline\underlinewithlessdepth
\makeatother

% --------------------------------------------------------------------------- %

\newcommand*\dbar[1]{\overline{\overline{#1}}}
% \newcommand*\dbar[1]{\overline{\overline{\lower0.2ex\hbox{$#1$}}}}
\newcommand{\harrow}[1]{\mathstrut\mkern2.5mu#1\mkern-11mu\raise1.6ex\hbox{$\scriptscriptstyle\rightharpoonup$}}
% \newcommand{\pirow}{{\pi^\star}}
\newcommand{\pirow}{\phi}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
% \def\eqref#1{equation~\ref{#1}}
% Ribeiro, more than one equation
\def\eqrefs#1#2{equations~\ref{#1} and~\ref{#2}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\eqref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
%\def\mA{\tA}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\expected}{\mathbb{E}}
\newcommand{\E}{\mathbb{E}} %....but this is a set in ICLR
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\ones}{\boldsymbol{1}}
\newcommand{\bpi}{\boldsymbol{\pi}}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\Loss}{\mathcal{L}}


% \NewDocumentCommand{\Prob}{o d()}{\ensuremath{
%     \mathds{P}[#1]
% }}


% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
%\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


% Jiasen:
\newcommand{\ea}{\emph{et al.}}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\iid}{\emph{i.i.d.}}
\newcommand{\wrt}{\emph{w.r.t.}\ }
\newcommand{\cf}{\emph{cf.}\ }

\newcommand{\ind}[1] {\mathbb{I}\{#1\}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Ab}{\mA}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\thetab}{\bm{\theta}}
%\newcommand{\grad}{\nabla}

\newcommand{\mix}[1]{\text{mix}\left(#1\right)}



==> outline.tex <==

*Causal graph

*Observational: what it gets wrong
  Increase the size, it impacts download time: Fig 4.
  
*Causal model:
    S depends on C. D depends on S and C.
    
Bring in Fig 6.

Possible Solution: Divide D by S.  [Throughput]
   If that were the case, just use throughput
   Not true because D depends on TCP state.
   Fig 5. Have a way to infer that. Not a simple equation anymore.
   
 TCP state depends on previous
 If you can add observable variables/block d-separate them, solution is simpler
 since you can look at current time rather than all time.
 
 Make Fig 7 a stack of time.. make this related.
 Observe download time, buffer time etc., blocks the path.. evolution of C 
 
 
 $C_t$ upto the time the current ABR is using it -> Interventional question
 $C_t$ for full trace using all data for the trace. -> Counterfactual question.
 
 Counterfactual: 
   If we used a different ABR that made different choices
   Change the first size: changing the 
   
   New ABR algoru
   
   ----
   Associational question: Given for that algorithm the past chunk sizes and download times were such and such, if the algorithm downloaded a chunk of this size, what would be the download time
   
   Counterfactual:Given a trace of a session with an existing ABR algorithm, replace with a new ABR algorithm, how does the new one perform
   
   Interventional: Existing traces with another ABR to improve the predictions of my new ABR 
                    
                    
    Biases that can occur:
    
    Consider Fugu.
    What it really wants is an interventional query: Task of a deployed algorithm is interventional:
    use that knowledge to improve the performance on a completely new session
    
    Fugu system: what it does is associational: it works if there are no confounders.
    
    What we are doing: get rid of confounders with HMM, then we can run with associational.
    
    Note for Bruno: Tom Mitchell's definition of learning.
